Understanding Innovation to Drive Sustainable Development

Innovation is among the key factors driving a country's economic and social growth. But what are the factors that make a country innovative? How do they differ across different parts of the world and different stages of development? In this work done in collaboration with the World Economic Forum (WEF), we analyze the scores obtained through executive opinion surveys that constitute the WEF's Global Competitiveness Index in conjunction with other country-level metrics and indicators to identify actionable levers of innovation. The findings can help country leaders and organizations shape the policies to drive developmental activities and increase the capacity of innovation.

==> correlations.tex <==
Before the analyses, we start by examining information captured in the WDI indicators. How comprehensive are they? How well do they portray a county? How well do they capture countries' differences and similarities? To obtain a better sense of the "story-telling" power captured in the WDI indicators, for each country in the dataset we compute its k-closest neighbors in the WDI feature spaces. We use $l_1$ distance (i.e. the Manhattan, or city block distance) as a measure of similarity, because it has been shown to be more robust and stable in capturing similarities in many practical applications than the Euclidian distance \citep{aggarwal2001surprising}. Table \ref{table:knn_wdi} shows examples of several countries and their five closest neighbors in the WDI space. As it can be seen from the examples, the WDI space captures the country level similarities well.

\begin{table*}
	\begin{center}
		\begin{tabular}{l l}
			
			\hline
			\textbf{Country} & \textbf{Top-5 Neighbors} \\ \hline
			\textbf￼{Canada} & Australia, Sweden, Austria, New Zealand, United Kingdom \\
			\textbf{Czech Republic} & Slovak Republic, Poland, Slovenia, Hungary, Austria \\
			\textbf{Sweden} & Finland, Denmark, Austria, Norway, Belgium \\
			\textbf{Kenya} & Tanzania, Uganda, Ghana, Mozambique, Cameroon \\
			\textbf{Japan} & France, Korea, Rep., Germany, United Kingdom, Canada \\
			\textbf{Nicaragua} & Honduras, El Salvador, Guatemala, Bolivia, Costa Rica \\ \hline
			
		\end{tabular}
	\end{center}
	\caption{Country level neighborhoods in WDI metrics space, and five closest neighbors for Canada, Czech Republic, Sweden, Kenya, Japan and Nicaragua.}
	\label{table:knn_wdi}
\end{table*}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{corrs.png}
	\caption{Top factors that 'universally' (i.e. in a majority of countries) correlate with perceived innovation output. Blue are positively correlated and red are negatively correlated.}
	\label{fig:corrs}
\end{figure}

As the first step towards understanding the innovation score and its relation to other country level indicators, we perform the basic correlation analysis to determine which WDI indicators rise with the rise in the innovation score and vice versa. Here, the innovation score refers to the overall 12th pillar innovation score in the GCI. We use the Pearson correlation coefficient method \citep{lee1988thirteen} to compute the correlation values. Figure \ref{fig:corrs} show the top positively and negatively correlated WDI indicators with the innovation score. Note that correlation analysis is performed at the global level (considering all countries). In that respect, the factors identified can be seen as representative of macro-level relationships, those that are "universally" related to innovation output (or at least observed in the majority of countries). We will explore more granular relationships between innovation score and metrics in subsequent section via predictive analyses.
